DecompGym: Benchmarking LLM Agents on Designing Decomposition Algorithms

Benders decomposition and column generation solve large optimization problems by passing cuts, columns, and dual values between a master problem and subproblems, and are hard to implement correctly. Large language models now automate parts of algorithm design, which points toward agents that build decomposition solvers for new problems. As a first step toward such agents, we study how well current coding agents design and implement these two algorithms, and how they fail. We introduce DecompGym, 81 instances from nine problem families (five Benders, four column generation), in which an agent writes a solver for a prescribed method. Each solver must meet three criteria: execution within a 60-second time limit; numerical feasibility together with a method audit, in which an LLM judge reads the solver's code; and an objective within 1% of the stored optimal objective. We evaluate 12 GPT, Claude, and Gemini models running in coding-agent tools. Over up to ten attempts, we compare independent regeneration with reflection, which first diagnoses the failure. On the first attempt, two models solve every instance and seven solve more than 90%. Most Benders failures (48 of 62) are missing or suboptimal solutions. The most common column-generation failure is a method-audit rejection. Output checks alone would accept 93 of the 108 attempts that fail the method audit. The most common rejection, an optimalif, occurs 96 times, 92 of them in one model.Reflection turns 66% of retries into successes, compared with 39% for regeneration, and it repairs method-audit failures, for which the judge names the defecective gaps. Agents for decomposition therefore need checks on how a solver reaches its answer and feedback that locates the error. The benchmark is available at https://github.com/SIKAI-C/DecompGym.

==> prompts/contract_benders.tex <==
Decomposition method requirements:

Use a master problem for the complicating decisions and recourse-cost estimates. Solve subproblems with the master decisions fixed, and use subproblem information to generate feasibility or optimality cuts and update subsequent master solves. Classical, integer, and logic-based Benders decomposition are allowed; LP duals are not required for integer or logic-based variants. Solving the master and fixed-decision subproblems as LPs or MIPs is allowed. Construct the reported solution from this decomposition, retaining a feasible incumbent when appropriate.


==> prompts/generation_csp.tex <==
Only edit the existing solver.py in the current working directory. All task context is supplied below.

Do not inspect other directories, use external tools or services, or search for reference implementations.

Do not execute the generated solver. The harness executes it later in its documented runtime directory.

Keep prose paragraphs and list items on one physical line; rely on editor soft wrapping.

You are an expert operations research engineer and Python programmer.

You are given a 1D cutting stock problem:
  - Stock length W = 247 cm.
  - Item types i=0..m-1, each with width size[i] and demand demand[i].
  - Objective: minimize number of stock pieces used.

Context: a manufacturing operation cutting stock material into ordered widths.

Input file data.json contains:
  - "stock_size" (or "roll_width"), "stock_unit"
  - "item_types": list of { "id": int, "name": str, "size": int, "demand": int }

Examples from this instance:
  - PaperProduct_0 (id=0, size=137, demand=41)
  - PaperProduct_1 (id=1, size=77, demand=35)
  - PaperProduct_2 (id=2, size=29, demand=60)
  - PaperProduct_3 (id=3, size=57, demand=29)
  - ...

Task:
Assume gurobipy and NumPy are available; the Python standard library is also allowed. Do not depend on any files other than data.json. Write a Python program solver.py that:
1) loads data.json,
2) Implements a Column Generation to solve the cutting stock problem,
3) writes output.json with at least:
{
  "status": "optimal | feasible | infeasible | error",
  "method": "column_generation",
  "objective_value": <#stock pieces used>,
  "solution": {
    "patterns": [
      {
        "pattern_id": <int>,
        "usage": <int>,
        "cuts": [
          {
            "item_id": <int>,
            "count": <int>
          },
          ...
        ]
      },
      ...
    ]
  }
}
Each pattern's total width must not exceed stock_size. Across all patterns (accounting for usage) every item demand must be met.

Decomposition method requirements:

Use a restricted master problem and pricing subproblems. Use master dual or reduced-cost information to generate columns, add useful columns to the restricted master, and reoptimize iteratively. A final integer solve of the restricted master over the accumulated columns is allowed. Construct the reported solution from this column-generation procedure.

Do not build and solve a separate monolithic optimization model of the full original problem, including for an initial incumbent, initialization, a warm start, a fallback, the reported solution, or an optimality certificate. This prohibition includes a full-original-model feasibility solve with a zero objective and applies to every reachable solution-producing path, including conditional fallback paths, even when decomposition also runs.

Heuristic initialization, directly constructed seed columns, phase-I restricted masters with artificial variables and pricing, valid initial bounds or cuts, and warm-starting a legitimate decomposition master are allowed. A permitted initialization must not obtain its solution from a separate full-original-model solve. The restriction concerns that separate full model, not legitimate decomposition masters, fixed-decision subproblems, pricing problems, or integer restricted masters.

Implement the information feedback required by the requested method. There is no minimum iteration count and no requirement that every instance add a cut or column, or improve the initial incumbent: legitimate immediate convergence or termination is allowed. Report mutually consistent decisions and objective values from the same incumbent. @@Use status feasible when returning an incumbent without a global optimality proof; optimality of an integer restricted master alone does not prove global optimality.@@

The data below are provided as read-only context for this editing call.
The generated solver.py will be executed later in a separate runtime directory, where it must read ../../data.json and write output.json in that runtime directory.

Implement a standalone solver.py using gurobipy, NumPy, and the Python standard library. Write output.json using the documented contract. Do not import repository implementations or load reference solutions.
The harness limits the entire solver.py execution to 60 seconds and numerical solvers to 1 thread(s). Design your algorithm and termination handling within this budget.

--- BEGIN CONTEXT: csp_medium_seed000/data.json ---
{
  "instance_size": "medium",
  "stock_size": 247,
  "stock_unit": "cm",
  "item_types": [
    {
      "id": 0,
      "name": "PaperProduct_0",
      "size": 137,
      "demand": 41
    },
    {
      "id": 1,
      "name": "PaperProduct_1",
      "size": 77,
      "demand": 35
    }
    <<elided: 4 more item types>>
  ]
}
--- END CONTEXT: csp_medium_seed000/data.json ---


==> prompts/judge.tex <==
Only edit the existing alg_verifier.md in the current working directory. All task context is supplied below.

Do not inspect other directories, use external tools or services, or search for reference implementations.

Do not execute the generated solver. The harness executes it later in its documented runtime directory.

Keep prose paragraphs and list items on one physical line; rely on editor soft wrapping.

Inspect the supplied solver.py and determine whether it implements column generation and substantively uses that method to produce the reported solution. Apply the following method contract, which is also supplied to the solver author:

Decomposition method requirements:

Use a restricted master problem and pricing subproblems. Use master dual or reduced-cost information to generate columns, add useful columns to the restricted master, and reoptimize iteratively. A final integer solve of the restricted master over the accumulated columns is allowed. Construct the reported solution from this column-generation procedure.

Do not build and solve a separate monolithic optimization model of the full original problem, including for an initial incumbent, initialization, a warm start, a fallback, the reported solution, or an optimality certificate. This prohibition includes a full-original-model feasibility solve with a zero objective and applies to every reachable solution-producing path, including conditional fallback paths, even when decomposition also runs.

Heuristic initialization, directly constructed seed columns, phase-I restricted masters with artificial variables and pricing, valid initial bounds or cuts, and warm-starting a legitimate decomposition master are allowed. A permitted initialization must not obtain its solution from a separate full-original-model solve. The restriction concerns that separate full model, not legitimate decomposition masters, fixed-decision subproblems, pricing problems, or integer restricted masters.

Implement the information feedback required by the requested method. There is no minimum iteration count and no requirement that every instance add a cut or column, or improve the initial incumbent: legitimate immediate convergence or termination is allowed. Report mutually consistent decisions and objective values from the same incumbent. @@Use status feasible when returning an incumbent without a global optimality proof; optimality of an integer restricted master alone does not prove global optimality.@@

Trace the entry point, relevant reachable call paths, information passed back to the master, and the code that writes output.json. Method names, comments, unused decomposition functions, or loops that do not feed subproblem information back into the master are insufficient. For an initialization or final solve, identify which decisions are fixed, which variables or columns are optimized, and where its result is used; an LP or MIP call by itself is not a violation.

Return FAIL if a reachable solution-producing path uses a prohibited separate full-original-model solve, even if decomposition also runs. For conditional fallbacks, cite the triggering conditions and role from source without assuming they ran. Unused helpers or provably unreachable branches alone are not a reason for FAIL. A genuine decomposition can converge or stop without adding a cut or column in a particular instance, and may return its initialized feasible incumbent.

This is an algorithm-use assessment, not a full mathematical proof of every cut, bound, or pricing formulation. Execution, feasibility, output consistency, and objective quality are checked separately. An incorrect numerical result alone is not a reason for algorithm FAIL; determine whether the requested decomposition is substantively implemented and used. Do not require a particular cut construction, initialization heuristic, pricing algorithm, or number of iterations.

Do not execute or modify solver.py. Do not claim to have observed runtime behavior when reviewing source only. Write alg_verifier.md with exactly a first line VERDICT: PASS or VERDICT: FAIL, followed by NOTES: and concise code evidence supporting the verdict.

--- BEGIN CONTEXT: attempt_01/solver.py ---
<<elided: 184 lines of attempt_01/solver.py>>
--- END CONTEXT: attempt_01/solver.py ---


==> prompts/judge_rationale_sonnet5.tex <==
VERDICT: FAIL
NOTES:
- The source substantively implements column generation: `main()` constructs single-item seed patterns, solves a continuous restricted master over `patterns`, passes demand-constraint duals (`c.Pi`) to a single-stock knapsack pricing problem, and appends a new pattern when its dual value exceeds `1.0 + 1e-6`; subsequent iterations rebuild and reoptimize the master with that column.
- Initialization directly constructs columns. The final integer master fixes each accumulated pattern's item counts and optimizes only its usage (`y_vars`). No separate full-original-model solve appears on any reachable path; time, iteration, master-status, and pricing termination paths proceed with the accumulated patterns.
- The explicit status/proof requirement is violated: `if final.Status == GRB.OPTIMAL: status = "optimal"` treats optimality of the integer restricted master as global optimality. This reachable branch requires no global bound comparison or other global proof, including after early column-generation termination. Such an incumbent must be reported as `feasible` unless global optimality is established.
- The successful `output.json` path derives pattern usages from `y_vars[p_idx].X` and the objective from their sum, but writes the unsupported `optimal` status above. The no-incumbent and exception paths write error results. This assessment is based solely on the supplied source; the solver was not executed.


==> prompts/quality_feedback.tex <==
The current solution is feasible, but its objective value does not meet the required target. Please try again.


==> prompts/reflection_advice_sonnet5.tex <==
# Debug Reflection -- attempt_01

## Diagnosis
The verifier failed the attempt on a single concrete defect: the final status-reporting logic conflates "integer restricted master solved to optimality" with "global optimality." The line `if final.Status == GRB.OPTIMAL: status = "optimal"` reports `optimal` whenever the final integer solve over the accumulated columns terminates optimally, but this only proves optimality of the restricted master (a subset of all possible cutting patterns), not of the original cutting-stock problem. Since the LP relaxation's column generation loop stops as soon as no column has reduced cost > 1 (i.e., LP-optimal for the restricted set), and the integer master is then solved separately, there is no global lower bound (e.g., ceil(LP relaxation objective) compared against the integer incumbent, or proof that no further columns could improve the integer solution) ever computed or checked. So the reported "optimal" status is unsupported -- everything else in the algorithm (seed patterns, dual-based knapsack pricing, iterative column addition, final integer solve) was judged structurally sound and compliant with the decomposition requirements.

## Root cause
Status assignment used local (restricted master) optimality as a proxy for global optimality without any certificate.

## Concrete changes for next attempt
1. Always report `status = "feasible"` for the incumbent produced by the final integer restricted-master solve, unless a genuine global optimality certificate is constructed (e.g., comparing the final integer objective to a valid lower bound such as ceil(final LP relaxation bound) AND confirming the pricing loop terminated because no improving column exists at the LP optimum, not merely because of a time/iteration cutoff).
2. Simplest compliant fix: unconditionally set `status = "feasible"` when returning any incumbent from the integer restricted master, since optimality of that integer program does not prove global optimality of the original cutting-stock problem (as stated explicitly in the task requirements). Only use `"optimal"` if the column-generation loop provably converged (no improving column exists, i.e., pricing objective <= 1 + tol) AND the final integer master's objective equals the LP relaxation's rounded-up bound -- otherwise default to `"feasible"`.
3. Keep all other logic (seed patterns, duals from master, knapsack pricing subproblem, final integer solve over accumulated columns) unchanged -- it already satisfies the decomposition requirements and avoids any monolithic full-model solve.
4. Double check: if `sub.Status == GRB.TIME_LIMIT` is used to break the loop (not a proven no-improving-column condition), that path must also report `"feasible"`, not `"optimal"`.


==> prompts/reflection_diagnosis.tex <==
<<the workspace rules of Prompt 1 with debug.md as the file to edit, the line "You are making an attempt to solve the following problem.", and the text of Prompt 1 from its first task line through its runtime rules>>

You have generated the solver.py file based on the problem description and the data.json file.
And the exec.log file shows the output of the solver.py file.
You also have alg_verifier.md with an LLM-based algorithm check; use it to improve the reflection.
Your tasks:
1) Read solver.py, exec.log, and the verifier feedback to diagnose execution, feasibility, algorithm, or objective-quality failures.
2) Write a concise reflection to debug.md: what likely went wrong and what the next attempt should change
3) List the concrete changes the next attempt should make in debug.md.
Keep the reflection concise and actionable.

--- BEGIN CONTEXT: csp_medium_seed000/data.json ---
<<elided: 42 lines of csp_medium_seed000/data.json>>
--- END CONTEXT: csp_medium_seed000/data.json ---

--- BEGIN CONTEXT: attempt_01/solver.py ---
<<elided: 184 lines of attempt_01/solver.py>>
--- END CONTEXT: attempt_01/solver.py ---

--- BEGIN CONTEXT: attempt_01/exec.log ---
<<elided: 16 lines of attempt_01/exec.log>>
--- END CONTEXT: attempt_01/exec.log ---

--- BEGIN CONTEXT: attempt_01/alg_verifier.md ---
<<elided: 6 lines of attempt_01/alg_verifier.md>>
--- END CONTEXT: attempt_01/alg_verifier.md ---

--- BEGIN CONTEXT: attempt_01/output.json ---
<<elided: 96 lines of attempt_01/output.json>>
--- END CONTEXT: attempt_01/output.json ---


==> prompts/revision_generation.tex <==
<<the generation instructions of Prompt 1, unchanged, followed by these context blocks>>

--- BEGIN CONTEXT: csp_medium_seed000/data.json ---
<<elided: 42 lines of csp_medium_seed000/data.json>>
--- END CONTEXT: csp_medium_seed000/data.json ---

--- BEGIN CONTEXT: attempt_01/solver.py ---
<<elided: 184 lines of attempt_01/solver.py>>
--- END CONTEXT: attempt_01/solver.py ---

--- BEGIN CONTEXT: attempt_01/debug.md ---
<<elided: 13 lines of attempt_01/debug.md>>
--- END CONTEXT: attempt_01/debug.md ---

